Mechanism Design with Predictions

Improving algorithms via predictions is a very active research topic in recent years. This paper initiates the systematic study of mechanism design in this model. In a number of well-studied mechanism design settings, we make use of imperfect predictions to design mechanisms that perform much better than traditional mechanisms if the predictions are accurate (consistency), while always retaining worst-case guarantees even with very imprecise predictions (robustness). Furthermore, we refer to the largest prediction error sufficient to give a good performance as the error tolerance of a mechanism, and observe that an intrinsic tradeoff among consistency, robustness and error tolerance is common for mechanism design with predictions.

==> app_frugal_ratio.tex <==
\section{Frugal Ratio}\label{sec:frugal_ratio}

==> app_proof.tex <==
\section{Omitted Proofs}\label{sec:omit_proof}

\subsection{Proof of \Cref{lem:auction_large_eta}}\label{sec:omit_auction_large_eta}




\subsection{Proof of \Cref{thm:auction_jump_point}}\label{sec:omit_auction_jump_point}



\subsection{Proof of \Cref{thm:auction_avg_ratio}}\label{sec:omit_auction_avg_ratio}


\subsection{Proof of \Cref{thm:path_auction_main}}\label{sec:omit_path_auction}





\subsection{Proof of \Cref{thm:path_auction_bound}}\label{sec:omit_path_auction_bound}

%\begin{proof}

%\end{proof}


\subsection{Proof of \Cref{thm:scheduling_main}}\label{sec:omit_scheduling}







\subsection{Proof of \Cref{thm:facility}}\label{sec:omit_facility}





